The Extended Littlestone's Dimension for Learning with Mistakes and Abstentions

This paper studies classification with an abstention option in the online setting. In this setting, examples arrive sequentially, the learner is given a hypothesis class $\mathcal H$, and the goal of the learner is to either predict a label on each example or abstain, while ensuring that it does not make more than a pre-specified number of mistakes when it does predict a label. Previous work on this problem has left open two main challenges. First, not much is known about the optimality of algorithms, and in particular, about what an optimal algorithmic strategy is for any individual hypothesis class. Second, while the realizable case has been studied, the more realistic non-realizable scenario is not well-understood. In this paper, we address both challenges. First, we provide a novel measure, called the Extended Littlestone's Dimension, which captures the number of abstentions needed to ensure a certain number of mistakes. Second, we explore the non-realizable case, and provide upper and lower bounds on the number of abstentions required by an algorithm to guarantee a specified number of mistakes.

==> backup.tex <==
\section{Outline}
This project is about online prediction with abstention. The problem is initially studied in the KWIK model~\cite{LLWS11, SZB10}.
We focus on the harder ``agnostic" case, dropping the assumption that there is an expert predicting perfectly.
Our goal is to provide nontrivial mistake and abstention tradeoffs in this setting.

Our contributions are as follows:
\begin{enumerate}
\item We prove that in the expert setting, under the $l$-mistake assumption~\cite{CBFHW96}, it is possible to design a master algorithm to make at most $l$ mistakes with a finite number of abstentions. To complement this result, we show that any algorithm guaranteeing at most $l-1$ mistakes must output an infinite number of abstentions.
\item We extend the idea to online classification with inifinite hypothesis classes. Under the assumption that the hypothesis class has finite Littlestone's dimension $d$, along with the $l$-mistake assumption, we show that it is possible to design an algorithm with at most $l+d$ mistakes, with a finite number of abstentions. To complement this result, we show that there exist a hypothesis class such that any algorithm guaranteeing at most $l+d-1$ mistakes must output an infinite number of abstentions.
\item We provide efficient algorithms for linear classification that is able to achieve nontrivial tradeoffs on mistakes and abstentions, partially answering a question by~\cite{DZ13}.
\item We give a conceptually simple weighted majority-style algorithm for the problem, extending the result of~\cite{LW94}.
\item We generalize the idea of mistake tree~\cite{L87} to online prediction with abstension case, and develop a similar notion, coined {\em Extended Littlestone's Dimension}.
\end{enumerate}

\section{Preliminaries}
We study the problem of online prediction with expert advice, where the learning algorithm is not only allowed to make predictions from $\{-1,1\}$, but also predict $\bot$(abstention). The goal is to provide a tradeoff between the mistakes and $\bot$ predictions. More concretely, suppose we are given a mistake budget $k$, we would like to output as few $\bot$'s as possible, subject to that the total number of mistakes is at most $k$. In particular, we consider the general {\em non-realizable} case, where there may not exist a perfect expert. This is in sharp contrast to the setting in~\cite{SZB10}, where realizablilty is explicitly assumed.

The interaction between the learner and the adversary goes as follows:\\
For $t = 1,2,\ldots,$:\\
\indent Receive experts' advice $(x_{1,t}, ... x_{N,t}) \in \cbr{-1,1}^N$.\\
\indent Make prediction $x_{A,t} \in \cbr{-1,1,\bot}$.\\
\indent Receive outome $y_t \in \cbr{-1,1}$.

We define the rounds of mistakes as $M = \{t: x_{A,t} = -y_t\}$ and the rounds of abstention as $D = \{t: x_{A,t} = \perp \}$.

\section{An Impossibility Result}
Suppose no assumptions are made on the expert advice $(x_{1,t}, ... x_{N,t})$ and the outcome $y_t$ for all $t$. Our first observation is, since we cannot make any guarantees about whether we will make a mistake at time $t$, no mistake bounds can be given. A natural assumption, already explored by~\cite{CBFHW96}, states that, there exists at least one expert that makes at most $l$ mistakes. In this setting, the results in~\cite{CBFHW96} can be equivalently rephrased as: with a mistake budget of $k = 2l + \sqrt{l\ln N} + \ln N$, there is an algorithm that makes at most $k$ mistakes and outputs $0$ $\bot$'s. \footnote{Moreover,~\cite{ALW06} states that if randomized prediction is allowed, the mistake budget can be even reduced to $l + \sqrt{l\ln N} + \ln N$.} Therefore a natural question is: is there any algorithm that works under a mistake budget strictly less than $k < 2l + \sqrt{l\ln N} + \ln N$, possibly at the price of using a number of $\bot$'s? We show that when $k \leq l-1$, it is impossible to derive such an algorithm.

\begin{theorem}
If $k = l-1$ and $N = 1$, then no deterministic algorithm can guarantee to make at most $k$ mistakes with a finite bound of $\bot$'s.
\end{theorem}

\begin{proof}
%We prove the statement for $k = l - 1$. The case $k < l - 1$ is implied by the result.
Consider the following strategy by the adversary: At time $t$, present experts' prediction $x_{1,t} = +1$ for all $t$; if the algorithm predicts $x_{A,t} = +1$, then reveal label $y_t = -1$; if $x_{A,t} = -1$, then reveal label $y_t = +1$; if $x_{A,t} = \perp$, then reveal label $y_t = +1$.

We prove the theorem by induction on $k$.

\textbf{Base Case:} For $k = 0$, $l = 1$, Suppose there is an algorithm $A$ that predicts with a finite number of abstentions over time. Consider the first time $t_0$ when it predicts $x_{A,t} \neq \bot$; By the advesary's strategy, expert 1 does not make a mistake at timesteps $1,2,\ldots,t_0 - 1$. Therefore at time $t_0$, when advesary reveals $y_t = -x_{A,t}$, the 1-mistake assumption is still maintained. Thus, $A$ is forced to make at least one mistake over time. 

\textbf{Inductive Case:} Suppose no deterministic algorithm can guarantee to make at most $k_0 - 1$ mistakes with a finite bound of $\bot$'s under $k_0$-mistake assumption. Then
Assume (for the sake of contradiction) there is an algorithm $A$ that makes $k_0$ mistakes with a finite bound of $\bot$'s under $k_0+1$ mistake assumption. Consider the first time $t_0$ when $A$ predicts $x_{A,t} \neq \bot$. By the adversary's strategy, $A$ makes a mistake at time $t_0$ and expert 1 makes at most one mistake in times $1,2,\ldots,t_0$. Thus from time $t_0 + 1$ onwards, the Algorithm $A$ makes at most $k_0 - 1$ mistakes under the $k_0$-mistake assumption, contradiction.
\end{proof}

\cz{Perhaps the result also holds for randomized algorithms?}

\section{An Algorithm based on Reduction to Realizable Case}
Our key observation is that under the $l$-mistake assumption, the standard conversion under BW algorithm can be readily applied here, reducing the agnostic problem to a realizable one. We remind the reader a version of~\cite{SZB10}'s algorithm, namely Algorithm~\ref{alg:szb} in Appendix. Its basic idea is that it keeps track of available mistake budget $m$ over time, with prediction given by a modified majority vote rule. If the fraction of experts predicting minority is above some threshold, it predicts abstention, otherwise it predicts the majority label.

We adopt the {\em conservative} principle, a standard simplification in the design of mistake bounded algorithms, in our reduction. That is, if the algorithm predicts a label $x_{A,t} \in \{-1, +1\}$, and it is correct (i.e. $x_{A,t} = y_t$), then it does not update its internal state. Therefore, without loss of generality, in each round $t$, we assume the algorithm either makes a mistake, or abstains from prediction. Formally, $t \in M$ or $t \in D$ for all $t$. %We call these rounds {\em nontrivial}.

\begin{algorithm}[H]
\caption{Reduction to Realizable Case}
\begin{algorithmic}[1]
\STATE Set $T_0 = \max\cbr{t: k + (k+1)[N \cdot {t \choose {\leq l}}]^{\frac{1}{k+1}} \geq t}$.
\STATE Initialization: error of experts $e_i \gets 0$,  $i \in \{1,2,\ldots,N\}$, nontrivial round counter $c \gets 0$, mistake budget $m \gets k$, total number of ``alive'' meta-experts $M \gets \sum_i {T_0 + 1 - c \choose {\leq l - e_i}}$.
\STATE Precalculate table $\cbr{G(M,m): 0 \leq M \leq N{T_0 + 1\choose {\leq l}}, 0 \leq m \leq k}$.
\FOR{$t=1,2,\ldots,$}
    \STATE {\em{\# Recalculate Optimal Threshold}} 
    \STATE Set $a^* = \max\cbr{0 \leq a \leq M/2: G(a, m-1) \leq G(M-a, m) }$.
    \STATE {\em{\# Make Prediction}} 
    \IF{$\sum_{i: x_{t,i} = -1} {T_0 - c \choose {\leq l - e_i}} + \sum_{i: x_{t,i} = +1} {T_0 - c \choose {\leq l - e_i - 1}} \leq a^*$}
    % This is the number of meta-experts remainingin the next round if y_t turns out to be -1
        \STATE predict $x_{A,t} = +1$.
    \ELSIF{$\sum_{i: x_{t,i} = +1} {T_0 - c \choose {\leq l - e_i}} + \sum_{i: x_{t,i} = -1} {T_0 - c \choose {\leq l - e_i - 1}} \leq a^*$}
        \STATE predict $x_{A,t} = -1$.
    \ELSE
        \STATE predict $x_{A,t} = \bot$.
    \ENDIF
    \STATE Receive feedback $y_t$.

    \STATE {\em{\# Internal State Update in Nontrivial Rounds}}  
 
    \IF{$x_{A,t} = -y_t$ or $\bot$}
        \FOR{$i = 1, 2, \ldots, N$}
            \STATE $e_i \gets e_i + 1$
        \ENDFOR
        \STATE $c \gets c + 1$
        \IF{$x_{A,t} = -y_t$}
            \STATE Update number of ``alive'' meta-experts $M \gets \sum_i {T_0 + 1 - c \choose {\leq l - e_i}}$.
            \STATE $m \gets m - 1$
        \ENDIF
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:reduction}
\end{algorithm}
\begin{theorem}
If there is an expert $i$ that makes at most $l$ mistakes over time, that is, $| \{t: y_t = x_{i,t} \} | \leq l$ and $k \geq l$, then Algorithm~\ref{alg:reduction} makes at most $k$ mistakes and at most $(2(k+1))^{\frac{k+1}{k-l+1}} N^{\frac{1}{k-l+1}}$ abstentions.
\label{thm:reduction}
\end{theorem}
\begin{proof}
We prove the theorem in three steps.

\cz{I realize that we can discuss the algorithmic procedure in two modules: the design of potential function $\Phi(S, c)$ (exponential weight/binomial weight), (finite expert class/infinite set of hypothesis) and the halving-style algorithm used(optimal dynamic programming/SZB10/non-adaptive threshold setting implicit in SZB10). This framework can generate $2\times 3 = 6$ different algorithms. }

\cz{Another simple proof is the following: define binomial potential function $\Phi(\cdot, \cdot)$ as:
\[ \Phi(S, c) = \sum_{i=1}^N {T_0 - c \choose {\leq l - e_i}} \]
where $S = \cbr{(x_1, y_1), \ldots, (x_t, y_t)}$, $e_i = \sum_{j=1}^t I(x_{i,t} \neq y_t)$. It satisfies the following three properties:\\
(1) Throughout, $\Phi$ maintains the following invariant:
\[ \Phi(S, c) \geq 1 \]
(2) Initially,
\[ \Phi(\emptyset, 0) = N {T_0 \choose {\leq l}} \]
(3) Relaxation:
\[ \Phi(S, c) \geq \Phi(S \cup \cbr{(x_{t+1}, -1)}, c+1) + \Phi( S \cup \cbr{(x_{t+1}, +1)}, c+1)\]
Another important potential function is the exponential potential
\[ \Phi(S, c) = \sum_{i=1}^N \beta^{e_i} (\frac{1}{1 + \beta})^c \]
which has the following three properties:\\
(1) Throughout, $\Phi$ maintains the following invariant:
\[ \Phi(S, c) \geq \beta^l (\frac{1}{1+\beta})^{T_0} \]
(The $\beta$ maximizing the RHS is that $\beta = \frac{l}{T_0 - l}$).\\
(2) Initially,
\[ \Phi(\emptyset, 0) = N \]
(3) Relaxation:
\[ \Phi(S, c) \geq \Phi(S \cup \cbr{(x_{t+1}, -1)}, c+1) + \Phi( S \cup \cbr{(x_{t+1}, +1)}, c+1)\]
We get that
\[ T_0 \leq k + (k+1) (\frac{\Phi(\emptyset, 0)}{\Phi(S, T_0)})^{\frac{1}{k+1}} \]
We can design a variant of Algorithm~\ref{alg:szb} that runs on top of such {\em potential functions}.
}

(1) Recall that without loss of generality, we assume all rounds $t$ are {\em nontrivial}, i.e. $t \in M \cup D$. We define the set of meta-experts by flipping at most $l$ predictions over a horizon of length $T_0+1$. For each expert $i$ with prediction at the first $T_0+1$ rounds $(x_1, \ldots, x_{T_0+1})$, define the associated set of meta-expert as
\[ E_i = \{(x_1, \ldots, x_{T_0+1}): |\{t \in [1, T_0 + 1]: x_t \neq x_{i,t}\}| \leq l \} \]
The set of meta-experts in consideration is defined as their union, i.e.: 
\[ \tilde{E} = \cup_{i=1}^N E_i \]
We show that Algorithm~\ref{alg:reduction} is equivalent to running Algorithm~\ref{alg:szb} on top of meta-experts $\tilde{E}$. On one hand, by the $l$-mistake assumption, at least one expert in $\tilde{E}$ makes no mistakes over time $1,2,\ldots,T_0+1$. On the other hand, at time $c$, the number of ``alive'' experts in $E_i$ (i.e. consistent with $(y_1, \ldots, y_c)$) is equal to the cardinality of
\[ \{(y_1, \ldots, y_c, x_{c+1}, \ldots, x_{T_0+1}): |\{t \in [c + 1, T_0 + 1]: x_t \neq x_{i,t}\}| \leq l - e_i \} \]
which is exactly ${T_0 - c + 1 \choose {\leq l - e_i}}$. Among them, the set of experts voting for label $x_{i, c+1}$ at time $c+1$ is
\[ \{(y_1, \ldots, y_c, x_{i, c+1}, x_{c+2} \ldots, x_{T_0+1}): |\{t \in [c + 2, T_0 + 1]: x_t \neq x_{i,t}\}| \leq l - e_i \} \]
of cardinality ${T_0 - c \choose {\leq l - e_i}}$;
the set of experts voting for label $-x_{i, c+1}$ at time $c+1$ is
\[ \{(y_1, \ldots, y_c, -x_{i, c+1}, x_{c+2} \ldots, x_{T_0+1}): |\{t \in [c + 2, T_0 + 1]: x_t \neq x_{i,t}\}| \leq l - e_i - 1\} \]
of cardinality ${T_0 - c \choose {\leq l - e_i - 1}}$.
Therefore the conditions in lines 5, 7 and 9 of Algorithm~\ref{alg:reduction} is the same as the condition in lines 4, 6 and 8 when running Algorithm~\ref{alg:szb} on top of $\tilde{E}$.

(2) We first show that the number of nontrivial rounds is at most $T_0$. Suppose the the sake of contradiction that the number of nontrivial rounds is at least $T_0 + 1$. Since the number of meta-experts at the beginning is $N {T_0 + 1 \choose {\leq l}}$, by Lemma~\ref{lem:szb}, running Algorithm~\ref{alg:szb} on top of meta-experts has the following guarantee:
\[ m \leq k \] 
\[ d \leq (k+1)(N {T_0 + 1 \choose {\leq l}} )^{\frac{1}{k+1}} \]
where $m = |M \cap [T_0 + 1]|$ and $d = |D \cap [T_0 + 1]|$. 

By the fact that all rounds are nonrivial, $m + d = T_0 + 1$, we get that
\[ T_0 + 1 \leq k + (k+1)(N {T_0 + 1 \choose {\leq l}} )^{\frac{1}{k+1}} \]
which contradicts with the definition of $T_0$.

(3) We give an upper bound on $T_0$. $T_0$ satisfies inequality
\[ T_0 \leq k + (k+1)(N \cdot {T_0 \choose {\leq l}})^{\frac{1}{k+1}} \]
Therefore,
\[ T_0 + 1 \leq \max(2(k+1), 2(k+1)(N \cdot {T_0 \choose {\leq l}})^{\frac{1}{k+1}}) \]
We consider two spearate cases.
\paragraph{Case 1: $T_0 \leq 2(k+1)$.} In this case we already have an upper bound on $T_0$.
\paragraph{Case 2: $T_0 > 2(k+1)$.}  Then, ${T_0 \choose \leq l} \leq (T_0 + 1)^l$, thus
\[ T_0 \leq 2(k+1)[N \cdot (T_0+1)^l]^{\frac{1}{k+1}} \]
Solving the inequality yields that
\[ T_0 \leq (2(k+1))^{\frac{k+1}{k-l+1}} N^{\frac{1}{k-l+1}} \]
Combining, we conclude that in both cases,
\[ T_0 \leq (2(k+1))^{\frac{k+1}{k-l+1}} N^{\frac{1}{k-l+1}} \]
\end{proof}
\cz{The bounds in the analysis is far from optimal. I suspect if we use the tightest form of SZB10, we can set a tighter $T_0$ which is the largest $t$ such that 
\[ t \leq k + ((k+1)! (N {T_0 \choose {\leq l}} )^{\frac{1}{k+1}}\] 
That is,
\[ (\frac{et}{k+1})^{k+1} \leq (\frac{et}{l})^l N \]
We get
\[ T_0 \leq \frac{1}{e} (k+1) (\frac{k+1}{l})^{\frac{l}{k+1-l}} N^{\frac{1}{k+1-l}} \leq (k+1) N^{\frac{1}{k+1-l}}\]
And I believe this bound is near-optimal when $k / l = 1 + o(1)$.
}


\cz{As a remark, the constants in the bound can be further tightened. Using the fact that $T \leq A + B$ implies $T \leq \max((1 + \epsilon)A, (1 + \frac{1}{\epsilon})B)$, we get that
\[ T_0 \leq \max((1 + \frac{1}{\epsilon})(k+1), ((1+\epsilon)(k+1))^{\frac{k+1}{k-l+1}} N^{\frac{1}{k-l+1}})\]
We can tune $\epsilon$ to optimize the bound subsequently. When $l = 0$, the leading coefficient of the second term can be tuned arbitrarily close to 1, matching~\cite{SZB10}.}


\section{Algorithms based on Weighted Majority}

\subsection{Agnostic Case}

\begin{algorithm}[H]
\caption{Weighted Majority Algorithm}
\begin{algorithmic}
\STATE Input: threshold $\gamma$, discount parameter $0 < \beta < 1$.
\STATE Initialization: $w_{i,t} = 1$ for all $i$.
\FOR{$t=1,2,\ldots,$}
    \IF{$\sum_{i: x_{t,i} = -1} w_{i,t} \leq  \gamma \sum_i w_{i,t}$}
        \STATE predict $x_{A,t} = +1$
    \ELSIF{$\sum_{i: x_{t,i} = +1} w_{i,t} \leq  \gamma \sum_i w_{i,t}$}
        \STATE predict $x_{A,t} = -1$
    \ELSE
        \STATE predict $x_{A,t} = \bot$
    \ENDIF
    \STATE Receive feedback $y_t$.
    \FOR{$i = 1,2,\ldots,N$}
        \IF{$x_{i,t} \neq y_t$}
            \STATE $w_{i,t} \gets \beta w_{i,t-1}$
        \ELSE
            \STATE $w_{i,t} \gets w_{i,t-1}$
        \ENDIF
    \ENDFOR
\ENDFOR
\end{algorithmic}
\label{alg:wm}
\end{algorithm}

\subsubsection{Mistake Bound Guarantees}

\begin{theorem}
Suppose there is an expert making at most $l$ mistakes. If $\gamma = \frac{1}{1+l}(\frac{1}{eN})^{\frac{1}{k+1-l}}$ and $\beta = \frac{l}{1+l}(\frac{1}{eN})^{\frac{1}{k+1-l}}$, then Algorithm~\ref{alg:wm} makes at most $k$ mistakes and at most $4.31 \frac{(k+1)(l+1)}{k+1-l} \ln(eN) (eN)^{\frac{1}{k+1-l}}$ $\bot$'s.
\end{theorem}
\begin{proof}
If $t \in M$, then $x_{A,t} = -y_t$, hence $\sum_{i: x_{i,t} = -x_{A,t}} w_{i,t} < \gamma \sum_i w_{i,t}$. Thus,
\[ \frac{\sum_i w_{i,t+1}}{\sum_i w_{i,t}} = \frac{\sum_{i: x_{i,t} = y_t} w_{i,t} + \beta \sum_{i: x_{i,t} = -y_t} w_{i,t}}{\sum_i w_{i,t}} = \frac{\sum_{i: x_{i,t} = -x_{A,t}} w_{i,t} + \beta \sum_{i: x_{i,t} = x_{A,t}} w_{i,t}}{\sum_i w_{i,t}} < \gamma + (1-\gamma)\beta \]
If $t \in D$, then both $\sum_{i: x_{i,t} = +1} w_{i,t} \geq \gamma \sum_i w_{i,t}$ and $\sum_{i: x_{i,t} = -1} w_{i,t} \geq \gamma \sum_i w_{i,t}$. Thus,
\begin{eqnarray*} 
&&\frac{\sum_i w_{i,t+1}}{\sum_i w_{i,t}} \\
&=& \frac{\sum_{i: x_{i,t} = y_t} w_{i,t} + \beta \sum_{i: x_{i,t} = -y_t} w_{i,t}}{\sum_i w_{i,t}} \\
&\leq& \max(\frac{\sum_{i: x_{i,t} = +1} w_{i,t} + \beta \sum_{i: x_{i,t} = -1} w_{i,t}}{\sum_i w_{i,t}}, \frac{\sum_{i: x_{i,t} = -1} w_{i,t} + \beta \sum_{i: x_{i,t} = +1} w_{i,t}}{\sum_i w_{i,t}}) \\
&\leq& \gamma\beta + (1-\gamma) 
\end{eqnarray*}
Therefore, the algorithm maintains the invariant that for any time $T$,
\begin{equation} 
\beta^l \leq \sum_i w_{i,t} \leq N (\gamma + (1- \gamma)\beta)^m \cdot (\gamma \beta + (1 - \gamma))^d 
\label{eqn:invwmagnostic}
\end{equation}
where $m = |M \cap [T]|$ is the number of mistakes and $d = D \cap [T]$ is the number of abstentions made upto time $T$.
\cz{Possible to set $\beta_1$, $\beta_2$ that depends on prediction / $\bot$?}

(1) Suppose $m \geq k+1$, then by Equation~\eqref{eqn:invwmagnostic},
\[ \beta^l \leq N (\beta + \gamma - \gamma\beta)^{k+1} \leq N (\beta + \gamma)^{k+1} \]
whereas by the setting of $\beta$ and $\gamma$, we have
\[ N (\beta + \gamma)^{k+1-l} (1 + \frac{\gamma}{\beta})^l = N ((\frac{1}{Ne})^{\frac{1}{k+1-l}})^{k+1-l} (1 + \frac{1}{l})^l < 1 \]
contradiction.

(2) By Equation~\eqref{eqn:invwmrealizable}, we also have
\[ \beta^l \leq N(\gamma \beta + (1 - \gamma))^d = N (1 - (1 - \beta) \gamma)^d \]
Therefore,
\begin{eqnarray*} 
d &\leq& \frac{l \ln\frac{1}{\beta} + \ln N}{\gamma (1 - \beta)} \\
&\leq& \frac{l (\ln (1 + \frac{1}{l}) + \frac{1}{k+1-l} \ln (eN) ) + \ln N}{(1-\frac{1}{e}) \frac{1}{e} \frac{1}{1+l} (\frac{1}{eN})^{\frac{1}{k+1-l}} } \\
&\leq& \frac{e^2}{e-1} \frac{(k+1)(l+1)}{k+1-l} \ln(eN) (eN)^{\frac{1}{k+1-l}} \\
&\leq& 4.31 \frac{(k+1)(l+1)}{k+1-l} \ln(eN) (eN)^{\frac{1}{k+1-l}}
\end{eqnarray*}

\end{proof}

\subsubsection{Improved Guarantees over Algorithms without Abstention}
\label{sub:improvedgrt}
\begin{lemma}
Let $\gamma \leq \frac{1}{6}$, $\beta \geq 0.7$, $a = \frac{\gamma}{1-\gamma}$ and $h = -\ln(\gamma + (1 - \gamma)\beta) \leq 0.5$. Then the number of mistakes made by Algorithm~\ref{alg:wm} is at most
\[ l(1 + a + ah) + \frac{\ln N}{h} \] 
and the number of abstentions made by Algorithm~\ref{alg:wm} is at most
\[ 2.4 \cdot \frac{l \ln 2 + \ln N}{a}\]
\end{lemma}

\begin{theorem}
Let $h = 0.5$ and $a = \sqrt{\frac{c\ln N}{4l}}$. Then the number of mistakes made by Algorithm~\ref{alg:wm} is at most
\[ l + \sqrt{cl\ln N}+ 2\ln N \] 
and the number of abstentions made by Algorithm~\ref{alg:wm} is at most
\[ 4.8 \cdot \sqrt{\frac{l}{c\ln N}} (l + \ln N)\]

\end{theorem}

\begin{theorem}
Let $c \geq 4$, $h = \sqrt{1/c}$ and $a = \frac{c\ln N}{l}$. Then the number of mistakes made by Algorithm~\ref{alg:wm} is at most
\[ l + (c + 2\sqrt{c}) \ln N \] 
and the number of abstentions made by Algorithm~\ref{alg:wm} is at most
\[ 2.4 \cdot \frac{l^2 \ln 2 / \ln N + l}{c}\]
\end{theorem}

We need a technical lemma, whose proof is by standard calculus.
\begin{lemma}
If $h \leq 0.5$ and $a \leq 0.2$, then
\[ \frac{-\ln(-ae^h + 1 + a)}{ah} \leq 1 + h \]
\end{lemma}


\section{Infinite Hypothesis Class}
\subsection{Extended Littlestone's Dimension}
\begin{definition}
The extended Littlestone's dimension of hypothesis class $\calH$ with a mistake budget $k$, $\ELdim(\calH,k)$, is defined recursively as:
\begin{eqnarray*} 
&& \ELdim(\calH, k)  \\
&=& \begin{cases} 0 & |\calH| = 1 \\ 1 + \max_x \min(\ELdim(V[(x,+1)], k-1), \ELdim(V[(x,-1)], k-1), \max(\ELdim(V[(x,+1)], k), \ELdim(V[(x,-1)], k)) & \text{o.w.}\end{cases} 
\end{eqnarray*}
\end{definition}
The extended Littlestone's dimension characterizes the number of nontrivial rounds \cz{Should we change the defn to ``the number of abstentions"?} if both the learner and the adversary plays optimally, given that the learner has mistake budget $k$ and the advesary is only allow to choose the underlying hypothesis from $\calH$.

\subsection{Examples}
\subsubsection{Thresholds}
Note that learning threshold classifiers $\calH$ is isomorphic to the problem of predicting with $|\calH|$ experts' advice. Therefore,
\[ \ELdim(\calH, k) = G(|\calH|, k) \]

\subsubsection{Unions of Singletons}
Consider the concept class of unions of at most $d$ singletons $\calH_d$, with instance domain $\calX$. Then,
\[ \ELdim(\calH_d, k) = \begin{cases} |\calX|-k & k \leq d \\ 0 & k = d \end{cases} \]

\subsubsection{Unions of Intervals}
Consider the concept class of unions of at most $d$ intervals $\calH_d$, with instance domain $\calX$. Then, we can upper bound the extended Littlestone's dimension as follows:
\[ \ELdim(\calH_d, k) \leq \begin{cases} |\calX| & 0 \leq k \leq 4d \\ 2 d |\calX|^{1/2} & 4d+1 \leq k \leq 6d \\ \ldots \\ l d |\calX|^{1/l} & 2ld + 1 \leq k \leq 2(l+1)d \end{cases} \]
\cz{I believe the dependence on $d$ can not be improved by much(but can be refined using Jensen's Inequality), since in the worst case it will be split into $d$ intervals of equal size and the adversary plays minimax optimally within each threshold learning problem.}

\subsection{Explanation via Extended Mistake Trees}
We use a tree to represent the advesary's strategy. Suppose we are in a subtree. Th adversary shows example $x_t$ to the learner and the learner makes prediction  $x_{A,t}$ in $\cbr{-1,+1,\bot}$. In response to the prediction, the adversary has the freedom to jump into the left branch(reveal $y_t = -1$ and plays consistent with $\calH[(x_t,-1)]$ subsequently), or jump into the right branch (reveal $y_t = +1$ and plays consistent with $\calH[(x_t,+1)]$ subsequently). Since only nontrivial rounds are considered, when $x_{A,t} = +1$, $y_t$ must be $-1$, and when $x_{A,t} = -1$, $y_t$ must be $+1$. We use solid lines to record these responses. On the other hand, when $x_{A,t} = \bot$, the adversary has the freedom to choose $y_t \in \cbr{-1,+1}$ as her wish. We use dashed lines to record these responses. When a leaf is reached, it must satisfy the condition that there exists a classifier in $\calH$ that is consistent with all the labelled examples along the path. Reaching a leaf means that the interaction between the learner and the adversary comes to an end. We call the resulting tree an {\em Extended Mistake Tree}.

\begin{figure}
\centering
\input{mistaketree.tex}
\caption{An illustration of a extended mistake tree.}
\end{figure}

Given an extended mistake tree, the goal of the learner can be reprased as to find the shortest path from the root to a leaf, using at most $k$ solid edges. That is, minimizing the number of nontrivial rounds, subject to that at most $k$ mistakes are incurred. In this view, the goal of the adversary is to construct an extended mistake tree such that every root to leaf path with at most $k$ solid edges is long enough.

As we will see, the construction of extended mistake trees will give us insights about lower bound of Extended Littlestone's dimension.

\subsubsection{Thresholds}

\paragraph{Base Case: $k = 0$.} The construction of the optimal extended mistake tree is in Figure~\ref{fig:thresholds}. It shows that $\ELdim(\calH) \geq |\calH| - 1$. We call the resulting tree $T(0,N-1)$.
\begin{figure}
\centering
\input{thresholds.tex}
\caption{An illustration of a extended mistake tree for the class of thresholds when $k = 0$.}
\label{fig:thresholds}
\end{figure}

\paragraph{General Case}
Let $d(k,a)$ be the smallest size of the tree such that all root to leaf paths with at most $k$ solid lines have length $a$.
We show by a specialized construction that
\[ d(k,a+1) \leq d(k-1,a) + d(k-1,a-1) + \ldots + d(k-1,1) + d(k-1,1) \]
\begin{figure}
\centering
\input{thresholdsgeneral.tex}
\caption{Construction of $T(k,a+1)$ from $T(k-1,a), \ldots, T(k-1,1)$.}
\label{fig:thresholdsgeneral}
\end{figure}
The recursive construction is in Figure~\ref{fig:thresholdsgeneral}: we can build a tree $T(k,a+1)$ such that all root to leaf paths with at most $k$ solid lines have length $a$, with size at most $|T(k-1,a)| + |T(k-1,a-1)| + \ldots + |T(k-1,1)| + |T(k-1,1)|$.

\begin{lemma}
\[ d(a,k) \leq \frac{a^{k+1}}{(k+1)!} \]
Hence
\[ \ELdim(\calH, k) \geq ((k+1)! |\calH|)^{\frac{1}{k+1}}\]
\end{lemma}

\subsubsection{Unions of Singletons}

We consider unions of singletons over an infinite domain $\calX$. That is, $\calH = \{I(x \in S) | S \subseteq \calX, |S| \leq d\}$. We show that the following dichotomy holds: 
\[ \ELdim(\calH, k) = \begin{cases} \infty & k < d \\ 0 & k = d \end{cases} \]
In particular, we show that it is possible to construct a mistake tree such that all of its finite paths have at least $d$ solid edges. Taking the contrapositive, any paths containing $<d$ edges must have length infinity, thus concluding the claim. 

\paragraph{Base Case: $d = 1$.} The case for $d = 1$ is the same as the construction in Figure~\ref{fig:thresholds}, except that when $|\calX|$ is infinity, the mistake tree can be extended to infinte depth.

\paragraph{General Case.} Consider the case when $d = l$. The construction is essentially the same as the construction in Figure~\ref{fig:thresholdsgeneral}. Alternatively, the strategy can be rephrased as: when the algorithm predicts abstention, the adversary always reveal the $-1$ label; otherwise the adversary reveals the label that is opposite to the learner's prediction. In this way, any learner cannot make at most $l-1$ mistakes with finite abstentions.

\begin{figure}
\centering
\input{unionsofsingletons.tex}
\caption{Construction of $T_l$ from $T_{l-1}$.}
\label{fig:unionsofsingletons}
\end{figure}

\subsection{Noisy Abstention Game using Hypothesis Class with Finite Littlestone's Dimension}
Suppose the Littlestone's dimension~\cite{L87, BPS09} of hypothesis class $\calH$ is $d$. Additionally let $l$ be an upper bound of the mistakes made by the best classifier in $\calH$. Then we have the following result.
\begin{lemma}
Suppose $\Ldim(\calH) = d$ and $k \geq l + d$. Define $T_0$ as 
\[ T_0 = \max\cbr{t: k + (k+1) \left( {t \choose {\leq d}} {t \choose {\leq l}} \right)^{\frac{1}{k+1}} \geq t} \]
Then there exists an algorithm working with $\calH$ that makes at most $k$ mistakes and $T_0$ $\bot$'s.
\end{lemma}
One algorithm that achieves this bound is by running the standard conversion $\Expert(i_1, \ldots, i_d)$, where $1 \leq i_1 \leq \ldots \leq i_{d_1} \leq T$ and $0 \leq d_1 \leq d$. It is shown in~\cite{BPS09} that the set of $T \choose {\leq d}$ experts completely simluates the predictions of all the hypotheses in $\calH$ for any input sequence $x_1, \ldots x_T$. Along with Lemma~\ref{lem:reduction}, we get the lemma above. 

Below we give a sometimes more efficient algorithm. Note this algorithm requires computing $\Ldim(V)$ for some version space $V$, which may still be intractable.

\begin{algorithm}[H]
\caption{A more efficient implementation}
\begin{algorithmic}
\STATE Set $T_0 = \max\cbr{t: k + (k+1)[{t \choose {\leq d}} \cdot {t \choose {\leq l}}]^{\frac{1}{k+1}} \geq t}$.
\STATE Initialization: nontrivial round counter $c \gets 1$, remaining mistake budget $m \gets k$, total number of meta-experts alive $M \gets {T_0 + 1 \choose {\leq d}} \cdot {T_0 + 1 \choose {\leq l}}$.
\FOR{$t=1,2,\ldots,$}
    \IF{$\sum_{\tilde{y}_1, \ldots \tilde{y}_t} {T_0 + 1 - c \choose \Ldim(H[(x_1,\tilde{y}_1), \ldots, (x_t,\tilde{y}_t)])} {T_0 + 1 - c \choose {\leq l - (\sum_{j=1}^{t-1}I(\tilde{y}_j \neq y_j) + I(\tilde{y}_t \neq 1))}} \leq M^{\frac{m}{m+1}}$}
        \STATE predict $x_{A,t} = 0$.
    \ELSIF{$\sum_{\tilde{y}_1, \ldots \tilde{y}_t} {T_0 + 1 - c \choose \Ldim(H[(x_1,\tilde{y}_1), \ldots, (x_t,\tilde{y}_t)])} {T_0 + 1 - c \choose {\leq l - (\sum_{j=1}^{t-1}I(\tilde{y}_j \neq y_j) + I(\tilde{y}_t \neq 0))}} \leq M^{\frac{m}{m+1}}$}
        \STATE predict $x_{A,t} = 1$.
    \ELSE
        \STATE predict $x_{A,t} = \bot$.
        \STATE $c \gets c + 1$
    \ENDIF
    \STATE Receive feedback $y_t$.

    \IF{$x_{A,t} \neq y_t$}
        \STATE $c \gets c + 1$
        \STATE $m \gets m - 1$
        \STATE Total number of meta-experts alive $M \gets \sum_{\tilde{y}_1, \ldots \tilde{y}_t} {T_0 + 1 - c \choose \Ldim(H[(x_1,\tilde{y}_1), \ldots, (x_t,\tilde{y}_t)])} {T_0 + 1 - c \choose {\leq l - (\sum_{j=1}^{t-1}I(\tilde{y}_j \neq y_j))}}$.
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:litreduction}
\end{algorithm}

\begin{lemma}
Suppose there is at least one expert $i$ that makes at most $l$ mistakes. Algorithm~\ref{alg:litreduction}, run on experts $x_t$ and feedbacks $y_t$, makes at most $k$ mistakes and $T_0$ abstensions.
\end{lemma}
\begin{proof}
Define potential function $\Phi(\cdot, \cdot)$ as:
\[ \Phi(\cbr{(x_1, y_1), \ldots, (x_t, y_t)}, c) = \sum_{\tilde{y}_1, \ldots, \tilde{y}_t} {T_0 - c \choose {\leq \Ldim(H[(x_1, \tilde{y}_1), \ldots, (x_t, \tilde{y}_t)])}} {T_0 - c \choose {\leq l - \sum_{j=1}^t I(y_t \neq \tilde{y}_t)}}\]
We know that by the $l$-mistake assumption, at any time $t$ and any nontrivial round counter $c \leq T_0$,
\[ \Phi(\cbr{(x_1, y_1), \ldots, (x_t, y_t)}, c) \geq 1 \]
whereas the initial potential is,
\[ \Phi_k = \Phi(\emptyset, 0) = {T_0 + 1 \choose {\leq d}} \cdot {T_0 + 1 \choose {\leq l}} \]
%The rest of the proof follows the same as Lemma~\ref{lem:szb}.
Another important property is that 
\[ \Phi(\cbr{(x_1, y_1), \ldots, (x_t, y_t)}, c) \geq \Phi(\cbr{(x_1, y_1), \ldots, (x_t, y_t), (x_{t+1}, 1)}, c + 1) + \Phi(\cbr{(x_1, y_1), \ldots, (x_t, y_t), (x_{t+1}, -1)}, c + 1)\]
Assume for the sake of contradiction that the number of nontrivial rounds is $T_0 + 1$. For $m \in [0,k]$, define epoch $m$ as the time steps $t$ when the mistake budget equals exactly $m$.

We first show that for all $m$, the number of alive experts at the beginning of epoch $m$, $\Phi_m$, is at most $\Phi_k^{\frac{m+1}{k+1}}$. At epoch $e$, if the algorithm makes a mistake, the number of remaining experts $M_{e-1}$ will be at most $M_e^{\frac{e}{e+1}}$. Hence,
\[ \Phi_m \leq (\Phi_{m+1})^{\frac{m+1}{m+2}} \leq ((\Phi_{m+2})^{\frac{m+2}{m+3}})^{\frac{m+1}{m+2}} \leq \ldots \leq ((\ldots(\Phi_k)^{\frac{k}{k+1}}\ldots)^{\frac{m+2}{m+3}})^{\frac{m+1}{m+2}} = \Phi_k^{\frac{m+1}{k+1}} \]

Fix $m$. We next show that the number of abstentions made throughout epoch $m$ is at most $\Phi_k^{\frac{1}{k+1}}$. Since every abstention eliminates at least $\Phi_m^{\frac{m}{m+1}}$ experts, the number of abstentions at epoch $m$ is at most
\[ \frac{\Phi_m}{\Phi_m^{\frac{m}{m+1}}} = \Phi_m^{\frac{1}{m+1}} \leq N^{\frac{1}{k+1}} \]

Therefore, the total number of abstentions is at most $d \leq \sum_{m=0}^k \Phi_k^{\frac{1}{k+1}} = (k+1) \Phi_k^{\frac{1}{k+1}} = (k+1)({T_0 + 1 \choose {\leq d}} \cdot {T_0 + 1 \choose {\leq l}})^{\frac{1}{k+1}}$. 
On the other hand, $m \leq k$, therefore,
\[ m + d = T_0 + 1 \leq k + (k+1)({T_0 + 1 \choose {\leq d}} \cdot {T_0 + 1 \choose {\leq l}})^{\frac{1}{k+1}} \]
which is a contradiction.
\end{proof}

\begin{lemma}
\[ T_0 \leq (2k+2)^{\frac{k+1}{k+1-d-l}} \]
\end{lemma}

\begin{proof}
$T_0$ satisfies inequality that
\[ T_0 \leq k + (k+1)({T_0 \choose {\leq d}} {T_0 \choose {\leq l}})^{\frac{1}{k+1}} \]
Therefore,
\[ T_0 + 1 \leq \max(2(k+1), 2(k+1)({T_0 \choose {\leq d} } {T_0 \choose {\leq l}})^{\frac{1}{k+1}}) \]
Suppose $T_0 \geq 2(k+1)$. Then, ${T_0 \choose \leq l} \leq (T_0 + 1)^l$ and ${T_0 \choose \leq d} \leq (T_0 + 1)^d$, thus
\[ T_0 \leq T_0 + 1 \leq 2(k+1)((T_0+1)^{l+d})^{\frac{1}{k+1}} \]
Solving the inequality yields that
\[ T_0 \leq (2(k+1))^{\frac{k+1}{k+1-l-d}} \]
\end{proof}


\paragraph{Remark.} The lemma above provides nontrivial tradeoffs between the number of mistakes and $\bot$ predictions. The paper~\cite{BPS09} discusses the case where there is not $\bot$ allowed. By using a conversion of Standard Optimal Algorithm~\cite{L87} and the Weighted Majority Algorithm~\cite{LW94, CFHHSW97, FS97}, they achieve a mistake bound of $l + \tilde{O}(\sqrt{l d \ln T} + d \ln T)$, where $T$ is the length of the horizon. In contrast, we show that when only $l + d$ mistakes are allowed, we are still able to get a nontrivial bound on the number of $\bot$'s.


\section{Efficient Algorithms for Linear Separators}

Consider the setting of linear prediction with side information.

\subsection{A Perceptron-style Algorithm}
\begin{algorithm}
\caption{Modified Perceptron}
\begin{algorithmic}
\STATE Initialization: $w_1 \gets 0$
\FOR{$t = 1,2...$}
    \STATE See example $x_t$.
    \IF{$|w_t \cdot x_t| \leq \alpha$}
        \STATE predict $\bot$
    \ELSE 
        \STATE predict $\sign(w_t \cdot x_t)$
    \ENDIF
    \STATE Receive feedback $y_t$.
    \IF{$y_t w_t \cdot x_t \leq \alpha$}
        \STATE update $w_{t+1} \gets w_t + \eta y_t x_t$
    \ELSE 
        \STATE $w_{t+1} \gets w_t$
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:paperceptron}
\end{algorithm}
We give a modified perceptron algorithm in the section. Note that the algorithm is {\em computationally efficient}, which does not require any reduction to expert algorithm. Define hinge loss $l_\gamma(\cdot, \cdot)$ as 
\[ l_\gamma(w, (x,y)) = (1 - y w x / \gamma)_+\]

\paragraph{Remark.} The algorithm can be straightforwardly extended to general mirror descent style linear classification algorithms. Suppose there is a Legendre function $R$ that is 1-strongly convex wrt norm $\| \cdot\|$ in domain $K$. The update can be modified as follows: $\nabla R(w_{t+1}) = \nabla R(w_{t+1}) + \eta y_t x_t$. Some canonical examples are:

1. $R(w) = B \sum_i w_i \ln w_i$ is 1-strongly convex wrt $\|\cdot\|_1$ in $K = \{w: w > 0 \wedge \|w\|_1 \leq B \}$, .

2. $R(w) = \frac{\|w\|_q^2}{2(q-1)}$ is 1-strongly convex wrt $\|\cdot\|_q$ in $K = \R^d$, for $q \in (1,2]$.

By standard result in online gradient descent, the regret can be characterized by
\[ \sum_t \langle w_t-u, z_t \rangle \leq \frac{R(u) - R(w_0)}{\eta} + \sum_t \frac{\eta \| z_t \|_*}{2} \]

Since a lot of analysis of perceptron follows from reduction to online linear optimization, other techniques, e.g. time-varying potentials (second order perceptron), local norm bounds(Bernstein bounds), can be easily generalized to this setting and similar mistake bounds can be derived.

\begin{theorem}
Suppose Algorithm~\ref{alg:paperceptron} has inputs the data sequence $(x_1,y_1), \ldots, (x_t, y_t)$, with $\|x_t\| \leq X_2$ for all $t$. 
Then for any $\delta \in (0, 1/2)$, there exists a settings of $\alpha$, $\eta$, such that for any vector $u$:\\
(1) The number of mistakes $m$ is at most
\[ \frac{1}{2 - 3\delta} (\sum_t l_\gamma(u, (x_t, y_t)) + \frac{X_2^2\| u \|^2}{2\delta\gamma^2}) \]
(2) The number of abstention $d$ is at most
\[ \frac{1}{\delta} (\sum_t l_\gamma(u, (x_t, y_t)) + \frac{X_2^2 \| u \|^2}{2\delta\gamma^2}) \]\\
\end{theorem}

\cz{Remark: Suppose $\delta = 0.01$. Then the number of mistake is about {\em half} of the hinge loss of the comparator $u$ on the sequence, plus some overhead on the complexity of hypothesis class. To the best of the authors' knowledge, the leading coefficient of hinge loss in the existing online learning literature is always at least $1$. We show that when abstention is allowed, new mistake bounds can be obtained.}

\begin{proof}
Note that the algorithm only makes an update in the nontrivial rounds $t \in M \cup D$. Therefore by standard result of online gradient descent~\cite{SS12}, we have that for any $u$,
\[ \sum_{t \in M \cup D} \langle w_t-u, -y_t x_t \rangle \leq \frac{\|u\|^2}{2\eta} + \sum_{t \in M \cup D} \frac{\eta\|x_t\|^2}{2} \]
That is,
\[ \sum_{t \in M \cup D} (\gamma - y_t w_t x_t - \frac{\eta\|x_t\|^2}{2}) \leq \frac{\|u\|^2}{2\eta} + \sum_{t \in M \cup D} (\gamma - y_t u x_t)  \]
Since $y_t w_t x_t \leq -\alpha$ when $t \in M$, and $y_t w_t x_t \leq \alpha$ when $t \in D$, we get that
\[ (\gamma + \alpha - \frac{\eta X_2^2}{2}) m + (\gamma - \alpha - \frac{\eta X_2^2}{2}) d \leq \frac{\|u\|^2}{2\eta} + \sum_{t \in M \cup D} (\gamma - y_t u x_t) \]
Setting $\alpha = (1 - 2\delta) \gamma$ and $\eta = \frac{2\delta\gamma}{X_2^2}$ yields that
\[ (2 - 3\delta) m + \delta d  \leq \frac{\|u\|^2 X_2^2 }{2\delta \gamma^2} + \sum_{t \in M \cup D} l_\gamma(u, (x_t, y_t)) \]
Thus proving the result.
\end{proof}

\subsection{A Winnow-style Algorithm and its Connection with Expert Problem}

\begin{algorithm}
\caption{Modified Winnow}
\begin{algorithmic}
\STATE Initialization: $w_1 \gets (1/N, \ldots, 1/N)$
\FOR{$t = 1,2...$}
    \STATE See example $x_t$.
    \IF{$|w_t \cdot x_t| \leq \alpha$}
        \STATE predict $\bot$
    \ELSE 
        \STATE predict $\sign(w_t \cdot x_t)$
    \ENDIF
    \STATE Receive feedback $y_t$.
    \IF{$y_t w_t \cdot x_t \leq \alpha$}
        \STATE update $w_{t+1,i} \gets w_{t,i} \exp(\eta y_t x_{t,i})$ for all $i$
        \STATE Normalize $w_{t+1} \gets w_{t+1} / Z_t$
    \ELSE 
        \STATE $w_{t+1} \gets w_t$
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:pawinnow}
\end{algorithm}

\begin{theorem}
Suppose Algorithm~\ref{alg:pawinnow} has inputs the data sequence $(x_1,y_1), \ldots, (x_t, y_t)$, with $\|x_t\|_{\infty} \leq X_\infty$ for all $t$. 
Then for any $\delta \in (0, 1/2)$, there exists a settings of $\alpha$, $\eta$, such that for any vector $u$:\\
(1) The number of mistakes $m$ is at most
\[ \frac{1}{2 - 3c\delta} (\sum_t l_\gamma(u, (x_t, y_t)) + \frac{X_\infty^2\ln N}{2\delta\gamma^2}) \]
(2) The number of abstention $d$ is at most
\[ \frac{1}{c\delta} (\sum_t l_\gamma(u, (x_t, y_t)) + \frac{X_\infty^2\ln N}{2\delta\gamma^2}) \]\\
\end{theorem}
%\begin{proof}
%Note that the algorithm only makes an update in the nontrivial rounds $t \in M \cup D$. Therefore by standard result of online gradient descent~\cite{SS12}, we have that for any $u$,
%\[ \sum_{t \in M \cup D} \langle w_t-u, -y_t x_t \rangle \leq \frac{\|u\|^2}{2\eta} + \sum_{t \in M \cup D} \frac{\eta\|x_t\|^2}{2} \]
%That is,
%\[ \sum_{t \in M \cup D} (\gamma - y_t w_t x_t - \frac{\eta\|x_t\|^2}{2}) \leq \frac{\|u\|^2}{2\eta} + \sum_{t \in M \cup D} (\gamma - y_t u x_t)  \]
%Since $y_t w_t x_t \leq -\alpha$ when $t \in M$, and $y_t w_t x_t \leq \alpha$ when $t \in D$, we get that
%\[ (\gamma + \alpha - \frac{\eta X_2^2}{2}) m + (\gamma - \alpha - \frac{\eta X_2^2}{2}) d \leq \frac{\|u\|^2}{2\eta} + \sum_{t \in M \cup D} (\gamma - y_t u x_t) \]
%Setting $\alpha = (1 - 2\delta) \gamma$ and $\eta = \frac{2\delta\gamma}{X_2^2}$ yields that
%\[ (2 - 3\delta) \gamma m + \delta \gamma d  \leq \frac{\|u\|^2 X_2^2 }{2\delta \gamma} + \sum_{t \in M \cup D} l_\gamma(u, (x_t, y_t)) \]
%Thus proving the result.
%\end{proof}

\begin{corollary}
Suppose Algorithm~\ref{alg:pawinnow} has inputs $(x_1,y_1), \ldots, (x_t, y_t)$, where $x_s \in \{-1,+1\}^N$ are the ``expert advice'' and $y_s \in \cbr{-1,+1}$ are the labels. Assume that there is an expert $i$ that makes at most $l$ mistakes, i.e. there is $i \in [N]$ such that $|\cbr{t: x_{i,t} \neq y_t}| \leq l$. Then for any $\delta > 0$, $c \in (0, 1/3\delta)$, there exists a settings of $\alpha = (1 - 2c\delta)\gamma$, $\eta = 2c\delta\gamma$, such that:\\
(1) The number of mistakes $m$ is at most
\[ l + 3cl\delta + \frac{\ln N}{2\delta} \]
(2) The number of abstention $d$ is at most
\[ \frac{1}{c\delta} (2l + \frac{\ln N}{2\delta}) \]
In particular, if $c \leq \frac{4l}{3\ln N}$ is a constant, setting $\delta = \sqrt{\frac{\ln N}{12 c l}}$ yields that 
\[ m \leq l + \sqrt{3cl\ln N}, \qquad d \leq \sqrt{\frac{12 l}{c\ln N}}(2l + \sqrt{3cl \ln N}) \]
Moreover, if $c' \leq \frac{2l}{\ln N}$ is a constant, setting $c = \frac{c'^2\ln N}{3l}$, $\delta = \frac{1}{2c'}$ yields that
\[ m \leq l + c' \ln N, \qquad d \leq \frac{6l}{c' \ln N} (2l + 2c' \ln N)\]
\end{corollary}
\cz{This basically gives a second proof of the results in Section~\ref{sub:improvedgrt}.}

\cz{This corollary has the interesting consequence that in our new model, it is possible to design a {\em deterministic} algorithm making at most $l + \sqrt{cl\ln N}$ mistakes, as opposed to $2l + \sqrt{2l\ln N}$ in~\cite{CBFHW96}. The improvement is significant if $l \gg \ln N$. This makes me wonder again: does randomized prediction provide better guarantees? What should be the randomized algorithm like?} 

\bibliographystyle{alpha}
\bibliography{agnostickwik}

\appendix
\section{Extended Discussion of Abstention Game in Realizable Case}
\subsection{Minimax Algorithm}
\begin{algorithm}[H]
\caption{Minimax Algorithm}
\begin{algorithmic}[1]
\STATE Initialization: mistakes each expert has made $e_i \gets 0$,  $i \in \{1,2,\ldots,N\}$, mistake budget $m \gets k$, total number of ``alive'' experts $M \gets N$.
\STATE Precalculate table $G(M,m): 0 \leq M \leq N, 0 \leq m \leq k$.
\FOR{$t=1,2,\ldots,$}
    \STATE {\em{\# Recalculate Optimal Threshold}} 
    \STATE Set $a^* = \max\cbr{0 \leq a \leq M/2: G(a, m-1) \leq G(M-a, m) }$.
    \STATE {\em{\# Make Prediction}} 
    \IF{$| \{i: x_{t,i} = -1 \wedge e_i = 0\} | \leq a^*$}
        \STATE predict $x_{A,t} = +1$.
    \ELSIF{$| \{i: x_{t,i} = +1 \wedge e_i = 0\} | \leq a^*$}
        \STATE predict $x_{A,t} = -1$.
    \ELSE
        \STATE predict $x_{A,t} = \bot$.
    \ENDIF
    \STATE Receive feedback $y_t$.

    \STATE {\em{\# State Update in Nontrivial Rounds}}  
 
    \IF{$x_{A,t} = -y_t$ or $\bot$}
        \FOR{$i = 1, 2, \ldots, N$}
            \STATE $e_i \gets e_i + 1$
        \ENDFOR
        \IF{$x_{A,t} = -y_t$}
            \STATE Update mistake budget $m \gets m - 1$
            \STATE Update total number of alive experts $M \gets | \{i: e_i = 0\} |$
        \ENDIF
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:szb}
\end{algorithm}

%\subsubsection{Connection between~\cite{SZB10} and Egg Dropping Game}
Let us first find the minimax value of abstension game in realizable case. Suppose $N$ experts are currently ``alive", and at most $k$ mistakes are allowed. We define function $G(N,k)$ as the number of nontrivial rounds, if both the learner and the adversary play optimally. Observe that 
\[ G(N, 0) = N - 1 \]
\[ G(N, k) = 0, 0 \leq N \leq 2^k \]
To derive an optimal strategy, it suffice to consider what would the adversary do at the first step. Since all $N$ experts are indistinguishable, it suffice to specify $a$, the number of experts predicting 1. Note that $0 \leq a \leq N$. Therefore,
\[ G(N, k) = \max_{0 \leq a \leq N} \min(G(a, k-1), G(N-a, k-1), \max(G(N, k), G(N-a, k))) + 1\]
This suggests that the minimax strategy of the learner is:
\[ x_{A,t} = \begin{cases} 1 & \text{$a \leq N/2$ and $G(a, k-1) \leq G(N-a,k)$} \\ -1 & \text{$a \geq N/2$ and $G(N-a,k-1) \leq G(a,k)$} \\ \bot & \text{otherwise}  \end{cases}\]


Since the RHS is symmetric for $0 \leq a \leq N/2$ and $N/2 \leq a \leq N$, we only need to consider one side, that is,
\begin{eqnarray*}
&& G(N, k) \\ 
&=& \max_{0 \leq a \leq N/2} \min(G(a, k-1), G(N-a, k-1), \max(G(N, k), G(N-a, k))) + 1\\
&=&  \max_{0 \leq a \leq N/2} \min(G(a, k-1), G(N-a, k)) + 1
\end{eqnarray*}

We define $a^*$, the $a$ that balances both terms in the minimand, as follows:
\[ a^* = \max\cbr{0 \leq a \leq N/2: G(a,k-1) \leq G(N-a,k)} \]

%Let $a^* = \min\cbr{0 \leq a \leq N/2: G(a, k-1) \geq G(N-a, k)}$. We claim that the $a^*$ achieves the maximum.
%We first show a simple lemma.
%\begin{lemma}
%\[ G(N-a^*, k) \geq G(a^*, k-1) -1 \]
%\end{lemma}
%\begin{proof}
%By definition of $a^*$,
%\[ G(N-a^*+1, k) \geq G(a^*-1, k-1) + 1 \]
%Meanwhile, 
%\[ G(N-a^*, k) \geq G(N-a^*+1, k-1) - 1 \]
%\[ G(a^*-1, k-1) \geq G(a^*, k-1) - 1 \]
%Combining the three inequalities concludes the proof.
%\end{proof}
%\begin{lemma}
%For any $0 \leq a \leq N/2$,  
%\begin{equation}
% \min(G(a, k-1), G(N-a, k)) \leq \min(G(a^*, k-1), G(N-a^*, k))
%\label{eqn:argmaxa}
%\end{equation}
%\end{lemma}
%\begin{proof}
%\textbf{Case 1: $a \leq a^* - 1$.} First by monotonicity,
%\[ G(a, k-1) \leq G(a^*, k-1)\]
%Secondly, 
%\[ G(a, k-1) \leq G(a^*-1, k-1) \leq G(N-a^*+1, k) - 1 \leq G(N-a^*, k) \]
%where the first inequaltiy is by monotonicity, the second inequality is by definition of $a^*$, and the third inequality is from the fact that $G(n+1,m) \leq G(n,m) + 1$ for positive integers $n$,$m$.
%Hence 
%\[ \min(G(a, k-1), G(N-a, k)) \leq G(a, k-1) \leq \min(G(a^*, k-1), G(N-a^*, k)) \]


%\textbf{Case 2: $a \geq a^* + 1$.}
%\[ G(N-a, k) \leq G(N-a^*, k) \leq G(a^*, k-1) \]
%Hence 
%\[ \min(G(a, k-1), G(N-a, k)) \leq G(N-a, k) \leq \min(G(a^*, k-1), G(N-a^*, k))\]

%In both cases, we see that Equation~\eqref{eqn:argmaxa} holds.

%\end{proof}
%Therefore, one of the minimax strategy for the adversary is to show the learner $a^*$ experts predicting 0, and $N-a^*$ experts predicting 1. When the predictor predicts $x_{A,t} = $ 0 or 1, the adversary reveals the label $y_t$ that is opposite to $x_{A,t}$. Otherwise when $x_{A,t} = \bot$, the adversary reveals label $y_t = 1$.

%On the other hand, since 
%\[ G(a, k-1) \geq G(N-a, k) \Leftrightarrow a \geq a^*\]
The minimax strategy for the learner can thus be summarized below:
\[ x_{A,t} = \begin{cases} \maj(x_{1,t}, \ldots, x_{N,t}) & \text{\#minority $\leq a^*$} \\ \bot & \text{\#minority $\geq a^*+1$}  \end{cases}\]

Curiously, one of the optimal strategies of the adversary is to show $a^*$ experts predicting 1. This is justified by the following lemma.
\begin{lemma}
\[ a^* \in \arg\max_{0 \leq a \leq N/2} \min(G(a, k-1), G(N-a, k)) \]
\end{lemma}
\begin{proof}

\end{proof}
Consider the following recurrence: 
\[ F(N,k) = \min_{0 \leq j \leq N/2} \max(F(j, k-1), F(N-j-1, k)) + 1 \]
\[ F(N, 0) = N - 1 \]
\[ F(N, k) = 0, 0 \leq N \leq 2^k \]

\begin{theorem}
$F(N,k) = G(N,k)$.
\end{theorem}
Curiously, the function $G$ has the following property. This again justifies the validity of $a^*$ as the threshold of abstention in majority vote.

\begin{lemma}
\[ a^* \in \arg\min_{0 \leq a \leq N/2} \max(G(a,k-1), G(N-a-1, k)) \]
\end{lemma}

\begin{proof}

\end{proof}
%\begin{proof}
%\textbf{Case 1: $a \leq a^* - 2$.} In this case, $G(a,k-1) \leq G(N-a, k) -1 \leq G(N-a-1,k)$. Hence, $\max(G(a, k-1), G(N-a-1, k)) = G(N-a-1,k)$. First, by monotonicity,
%\[ G(N-a-1,k) \geq G(N-a^*, k) \]
%Secondly,
%\[ G(N-a-1,k) \geq G(N-a^*+1, k) \geq G(a^*-1, k-1)\]
%where the first inequality is by monotonicity, the second inequality is by the definition of $a^*$. Therefore, the inequality holds.


%\textbf{Case 2: $a \geq a^*$.} In this case, $G(a,k-1) \geq G(N-a,k) \geq G(N-a-1,k)$. Hence $\max(G(a, k-1), G(N-a-1, k)) = G(a,k-1)$. First by monotonicity,
%\[ G(a, k-1) \geq G(a^*-1, k-1) \]
%Secondly,
%\[ G(a, k-1) \geq G(a^*, k-1) \geq G(N-a^*, k) \]
%where the first inequality is by monotonicity, the second inequality is by the definition of $a^*$. Therefore, the inequality holds.

%In summary, the inequality holds in both cases.
%\end{proof}


%Consider the realizable case. Suppose $N$ experts are currently ``alive", and at most $k$ mistakes are allowed subsequently. Consider the following voting prediction rule:
%\[ x_{A,t} = \begin{cases} \maj(x_{1,t}, \ldots, x_{N,t}) & \text{\#minority $\leq a$} \\ \bot & \text{otherwise}  \end{cases}\]
%where $a$ is a tuning parameter depending on $N$. Denote by $F(N,k)$ the number of $\bot$'s that the algorithm using optimal setting of $a$ makes, we get the following recurrence:
%\[ F(N,k) = \min_{0 \leq a \leq N} \max(F(N-a, k) + 1, F(a, k-1))\]
%\[ F(1,k) = 0\]
%\[ F(N,0) = \infty (N \geq 2)\]
%Note that $a$ can be chosen from $[0,N]$, as opposed to $[0,N/2]$. If the optimal $a$ is greater than $N/2$, this indicates that for some setting $k$ and $N$, the algorithm may simply predict the majority label, irrespective of the prediction of each experts. 

%Fix $a$. By unrolling the first term repeatedly, it can be seen that
%\begin{eqnarray*} 
%F(N,k) &\leq& \max(F(N-a, k) + 1, F(a, k-1)) \\ 
%&\leq& \max(F(N-2a, k) + 2, F(a, k-1)+1, F(a, k-1)) \\
%&\leq&\ldots\\ 
%&\leq& \frac{N}{a} + F(a,k-1) 
%\end{eqnarray*}
%We can thus prove by induction that $F(N, k) \leq (k+1)N^{\frac{1}{k+1}}$. More interestingly this recovers Algorithm 2 of~\cite{SZB10}, since the threshold $a$ set in the proof is equal to $N^{\frac{k}{k+1}}$.



\subsection{A Slightly Refined Version of~\cite{SZB10}'s Algorithm}
\subsubsection{A Rough Estimate of $G(N,k)$}
Recall that 
\[ G(N,k)= \min_j \max (G(j-1, k-1), G(N-j, k)) + 1 \]
\[ G(N,0) = N-1 \]
We derive an analytical upper bound of $G(N,k)$, refining the result of~\cite{GF08,SZB10}. \cz{The result in~\cite{GF08} is not very accurate since the choice of first move is not an integer.}
\begin{theorem}
\[ G(N,k) \leq (k+1) N^{\frac{1}{k+1}} \]
\end{theorem}
\begin{proof}
Fix $j = \lceil N^{\frac{k}{k+1}} \rceil$ or $j = \lfloor N^{\frac{k}{k+1}} \rfloor + 1$. Note that $j - 1 \leq N^{\frac{k}{k+1}}$, and $j \geq N^{\frac{k}{k+1}}$.
\begin{eqnarray*} 
&& G(N,k) \\
&\leq& \max (G(j-1, k-1)+1, G(N-j, k)+1) \\
&\leq& \max (G(j-1, k-1)+1, G(j-1, k-1)+2, G(N-j, k)+2) \\
&\leq& \ldots \\
&\leq& \max (G(j-1, k-1)+1, G(j-1, k-1)+2, \ldots, G(j-1, k-1)+\lfloor \frac{N}{j} \rfloor, G(N-j \lfloor \frac{N}{j} \rfloor, k)+\lfloor \frac{N}{j} \rfloor) \\
&=& \max(G(j-1, k-1), G(N-j \lfloor \frac{N}{j} \rfloor, k)) + \lfloor \frac{N}{j} \rfloor \\
&\leq& G(j-1,k-1) + \lfloor \frac{N}{j} \rfloor \\
&\leq& G(N^{\frac{k}{k+1}}, k-1) + N^{\frac{1}{k+1}}
\end{eqnarray*}
The bound on $G$ can thus be concluded by induction on $k$.
\end{proof}

\subsubsection{The Algorithm}


\begin{algorithm}[H]
\caption{A Slightly Refined Version of~\cite{SZB10}'s Algorithm}
\begin{algorithmic}[1]
\STATE Initialization: mistakes each expert has made $e_i \gets 0$,  $i \in \{1,2,\ldots,N\}$, mistake budget $m \gets k$, total number of ``alive'' experts $M \gets N$.
\FOR{$t=1,2,\ldots,$}
    \STATE {\em{\# Make Prediction}} 
    \IF{$| \{i: x_{t,i} = -1 \wedge e_i = 0\} | \leq \lceil M^{\frac{m}{m+1}} \rceil-1$}
        \STATE predict $x_{A,t} = +1$.
    \ELSIF{$| \{i: x_{t,i} = +1 \wedge e_i = 0\} | \leq \lceil M^{\frac{m}{m+1}} \rceil-1$}
        \STATE predict $x_{A,t} = -1$.
    \ELSE
        \STATE predict $x_{A,t} = \bot$.
    \ENDIF
    \STATE Receive feedback $y_t$.

    \STATE {\em{\# State Update in Nontrivial Rounds}}  
 
    \IF{$x_{A,t} = -y_t$ or $\bot$}
        \FOR{$i = 1, 2, \ldots, N$}
            \STATE $e_i \gets e_i + 1$
        \ENDFOR
        \IF{$| \{i: e_i = 0\} | \leq \lfloor M^{\frac{m}{m+1}} \rfloor$}
            \STATE Update mistake budget $m \gets m - 1$
            \STATE Update total number of alive experts $M \gets | \{i: e_i = 0\} |$
        \ENDIF
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:szb}
\end{algorithm}

\begin{lemma}[Slightly Improves~\cite{SZB10}]
If there is an expert $i$ that makes no mistakes, that is $y_t = x_{i,t}$ for all $t$. Then Algorithm~\ref{alg:szb}, run with the $N$ experts, makes at most $k$ mistakes and has $(k+1)N^{\frac{1}{k+1}}$ nontrivial rounds.
\label{lem:szb}
\end{lemma}
\begin{proof}
For $m \in [0,k]$, define epoch $m$ as the time steps $t$ when the mistake budget equals exactly $m$.

We first show that for all $m$, the number of alive experts at the beginning of epoch $m$, $M_m$, is at most $N^{\frac{m+1}{k+1}}$. First by definition, $M_k = N$. At the start of epoch $e-1$, the number of remaining experts $M_{e-1}$ is at most $\lfloor M_e^{\frac{e}{e+1}} \rfloor$. Hence,
\[ M_m \leq (M_{m+1})^{\frac{m+1}{m+2}} \leq ((M_{m+2})^{\frac{m+2}{m+3}})^{\frac{m+1}{m+2}} \leq \ldots \leq ((\ldots(M_k)^{\frac{k}{k+1}}\ldots)^{\frac{m+2}{m+3}})^{\frac{m+1}{m+2}} = N^{\frac{m+1}{k+1}} \]

Fix $m$. We next show that the number of nontrivial rounds throughout epoch $m$ is upper bounded by $\lfloor M_m^{\frac{1}{m+1}} \rfloor$, which is at most $N^{\frac{1}{k+1}}$. Assume for the sake of contradiction that the number of nontrivial rounds is at least $\lfloor M_m^{\frac{1}{m+1}} \rfloor + 1$. If there is a mistake, then it must appear in the last round. Therefore, there must be $\lfloor M_m^{\frac{1}{m+1}} \rfloor$ consecutive abstensions before an abstention or a mistake, making the number of experts already at most 
\[ M_m - \lfloor M_m^{\frac{1}{m+1}} \rfloor (\lfloor M_m^{\frac{m}{m+1}} \rfloor + 1) \leq M_m - \lfloor M_m^{\frac{1}{m+1}} \rfloor M_m^{\frac{m}{m+1}} \leq  M_m^{\frac{m}{m+1}}  \] 
Therefore, the total number of nontrivial rounds is at most $\sum_{m=0}^k N^{\frac{1}{k+1}} = (k+1) N^{\frac{1}{k+1}}$. 
\end{proof}

\subsection{Generalized Halving Algorithm}

\begin{algorithm}[H]
\caption{Halving Algorithm}
\begin{algorithmic}
\STATE Input: threshold $\gamma$.
\STATE Initialization: $w_{i,t} = 1$ for all $i$.
\FOR{$t=1,2,\ldots,$}
    \IF{$\sum_{i: x_{t,i} = -1} w_{i,t} < \gamma \sum_i w_{i,t}$}
        \STATE predict $x_{A,t} = +1$
    \ELSIF{$\sum_{i: x_{t,i} = +1} w_{i,t} < \gamma \sum_i w_{i,t}$}
        \STATE predict $x_{A,t} = -1$
    \ELSE
        \STATE predict $x_{A,t} = \bot$
    \ENDIF
    \STATE Receive feedback $y_t$.
    \FOR{$i = 1,2,\ldots,N$}
        \IF{$x_{i,t} \neq y_t$}
            \STATE $w_{i,t} \gets 0$
        \ELSE
            \STATE $w_{i,t} \gets w_{i,t-1}$
        \ENDIF
    \ENDFOR
\ENDFOR
\end{algorithmic}
\label{alg:halving}
\end{algorithm}

We first present a simple algorithm, namely Algorithm~\ref{alg:halving} that achieves near-optimal mistake/abstention tradeoffs.
\begin{theorem}
Suppose there is an expert making no mistakes. If $\gamma = (\frac{1}{N})^{\frac{1}{k+1}}$, then Algorithm~\ref{alg:halving} makes at most $k$ mistakes, and has at most $N^{\frac{1}{k+1}} \ln N$ nontrivial rounds.
\end{theorem}
\begin{proof}
If $t \in M$, then $x_{A,t} = -y_t$, hence $\sum_{i: x_{i,t} = -x_{A,t}} w_{i,t} < \gamma \sum_i w_{i,t}$. Thus,
\[ \frac{\sum_i w_{i,t+1}}{\sum_i w_{i,t}} = \frac{\sum_{i: x_{i,t} = y_t} w_{i,t}}{\sum_i w_{i,t}} = \frac{\sum_{i: x_{i,t} = -x_{A,t}} w_{i,t}}{\sum_i w_{i,t}} < \gamma \]
If $t \in D$, then both $\sum_{i: x_{i,t} = +1} w_{i,t} \geq \gamma \sum_i w_{i,t}$ and $\sum_{i: x_{i,t} = -1} w_{i,t} \geq \gamma \sum_i w_{i,t}$. Thus,
\[ \frac{\sum_i w_{i,t+1}}{\sum_i w_{i,t}} = \frac{\sum_{i: x_{i,t} = y_t} w_{i,t}}{\sum_i w_{i,t}} \leq \max(\frac{\sum_{i: x_{i,t} = +1} w_{i,t}}{\sum_i w_{i,t}}, \frac{\sum_{i: x_{i,t} = -1} w_{i,t}}{\sum_i w_{i,t}}) \leq 1-\gamma \]
Therefore, the algorithm maintains the invariant that for any time $T$,
\begin{equation} 
1 \leq |\{i: e_i = 0\}| = \sum_i w_{i,T} \leq N \gamma^m (1- \gamma)^d 
\label{eqn:invwmrealizable}
\end{equation}
where $m = | [T] \cap M |$ is the number of mistakes and $d = |[T] \cap D|$ is the number of abstentions made upto time $T$.

(1) Suppose $m \geq k+1$, then by Equation~\eqref{eqn:invwmrealizable},
\[ 1 \leq N \gamma^m \leq N \gamma^{k+1} < 1\]
contradiction. Thus $m \leq k$.
\cz{The equation is slightly off -- $<$ vs. $\leq$}

(2) By Equation~\eqref{eqn:invwmrealizable}, we have
\[ 1 \leq N(1- \gamma)^{m+d} \leq N e^{-\gamma (m + d)} \]
Therefore,
\[ m + d \leq \frac{\ln N}{\gamma} = N^{\frac{1}{k+1}} \ln N \]
\end{proof}

\section{A Generalization of~\cite{SZB10}'s Algorithm}
\begin{algorithm}[H]
\caption{A Generalization of~\cite{SZB10}'s Algorithm}
\begin{algorithmic}[1]
\STATE Input: potential function $\Phi$, potential lower bound $p$.
\STATE Initialization: examples in the nontrivial rounds $S \gets \emptyset$, Nontrivial round counter $c \gets 0$, mistake budget $m \gets k$, current potential ratio $M \gets \Phi(\emptyset,0) / p$.
\FOR{$t=1,2,\ldots,$}
    \STATE {\em{\# Make Prediction}} 
    \IF{$\Phi(S \cup \cbr{(x_t, -1)}, c+1) \leq M^{\frac{m}{m+1}} \Phi(S, c)$}
        \STATE predict $x_{A,t} = +1$.
    \ELSIF{$\Phi(S \cup \cbr{(x_t, +1)}, c+1) \leq M^{\frac{m}{m+1}} \Phi(S, c)$}
        \STATE predict $x_{A,t} = -1$.
    \ELSE
        \STATE predict $x_{A,t} = \bot$.
    \ENDIF
    \STATE Receive feedback $y_t$.

    \STATE {\em{\# State Update in Nontrivial Rounds}}  
 
    \IF{$x_{A,t} = -y_t$ or $\bot$}
        \STATE Examples seen $S \gets S \cup \cbr{(x_t, y_t)}$.
        \STATE Nontrivial round counter $c \gets c + 1$.
    \ENDIF
    \IF{$x_{A,t} = -y_t$}
        \STATE Potential Ratio $M \gets \Phi(S, c) / p$.
    \ENDIF
\ENDFOR
\end{algorithmic}
\label{alg:szb}
\end{algorithm}

